On the Discrete Fr\'echet Distance in a Graph

The Fr\'{e}chet distance is a well-studied similarity measure between curves that is widely used throughout computer science. Motivated by applications where curves stem from paths and walks on an underlying graph (such as a road network), we define and study the Fr\'{e}chet distance for paths and walks on graphs. When provided with a distance oracle of $G$ with $O(1)$ query time, the classical quadratic-time dynamic program can compute the Fr\'{e}chet distance between two walks $P$ and $Q$ in a graph $G$ in $O(|P| \cdot |Q|)$ time. We show that there are situations where the graph structure helps with computing Fr\'{e}chet distance: when the graph $G$ is planar, we apply existing (approximate) distance oracles to compute a $(1+\varepsilon)$-approximation of the Fr\'{e}chet distance between any shortest path $P$ and any walk $Q$ in $O(|G| \log |G| / \sqrt{\varepsilon} + |P| + \frac{|Q|}{\varepsilon } )$ time. We generalise this result to near-shortest paths, i.e. $\kappa$-straight paths, as we show how to compute a $(1+\varepsilon)$-approximation between a $\kappa$-straight path $P$ and any walk $Q$ in $O(|G| \log |G| / \sqrt{\varepsilon} + |P| + \frac{\kappa|Q|}{\varepsilon } )$ time. Our algorithmic results hold for both the strong and the weak discrete Fr\'{e}chet distance over the shortest path metric in $G$. Finally, we show that additional assumptions on the input, such as our assumption on path straightness, are indeed necessary to obtain truly subquadratic running time. We provide a conditional lower bound showing that the Fr\'{e}chet distance, or even its $1.01$-approximation, between arbitrary \emph{paths} in a weighted planar graph cannot be computed in $O((|P|\cdot|Q|)^{1-\delta})$ time for any $\delta > 0$ unless the Orthogonal Vector Hypothesis fails. For walks, this lower bound holds even when $G$ is planar, unit-weight and has $O(1)$ vertices.

==> disttable.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c c c c c c c c c }
\textnormal{dist.} & \redvertex $\alpha$ & \redvertex $\alpha^\ast$ & 
\redvertex $\beta$ & \redvertex $\beta^{\ast}$ & \redvertex $\gamma$ & \redvertex $A^{\{ 0 \} }$ & \redvertex $A^{\{ 1 \} }$ & \redvertex $A$\\
%& \alpha & \alpha^\ast & \beta & \beta^{\ast} & \gamma & A^0 & A^1, A\\
\bluevertex x & \nearvertex .65 & \nearvertex 2.65 & \nearvertex 2.3 & \farvertex 4.3 & \nearvertex 2.702 & \nearvertex 2.301 & \nearvertex  2.951 & \nearvertex  2.952\\
\bluevertex y & \nearvertex 1.6 & \farvertex 3.6 & \nearvertex 2.601 & \farvertex 4.601 & \nearvertex 2.952 & \farvertex 3.251 & \farvertex 3.302 & \farvertex 3.202\\
\bluevertex z & \nearvertex 2.3 & \farvertex 4.3 & \nearvertex .65 & \nearvertex 2.65 & \nearvertex 1.652 & \nearvertex 0.652 & \nearvertex 1.302 & \nearvertex 1.652 \\
\bluevertex $B^{\{ 0 \} }$ & \nearvertex 1.95 & \farvertex 3.95 & \nearvertex \nearvertex 2.3 & \farvertex 4.3 & \farvertex 3.301 & \nearvertex 2.301 & \nearvertex 2.951 & \farvertex 3.301\\
\bluevertex $B^{\{ 1 \} }$ & \nearvertex 1.7 & \farvertex 3.7 & \nearvertex 2.701 & \farvertex 4.701 & \farvertex 3.051 & \nearvertex 2.951 & \farvertex 3.402 & \farvertex 3.302\\
\bluevertex B & \nearvertex 1.35 & \farvertex 3.35 & \nearvertex 2.351 & \farvertex 4.351 & \nearvertex 2.702 & \farvertex 3.001 & \farvertex 3.051 & \nearvertex 2.951\\
    \end{tabular}
    \caption{The shortest distance between vertices with a label in \colorbox{red!20}{$\{ \alpha, \alpha^*, \beta, \beta^*, \gamma, \Az, \Ao, A \}$} and in \colorbox{blue!20}{\{ x, y, z, \Bz, \Bo, B \}}, showing \colorbox{gray!05}{far} and \colorbox{yellow!20}{near} pairs of labels.}
    \label{tab:my_label}
\end{table}



% Old version:
%x & .65 & 2.65 & 1.95 & \cellcolor{gray!20} 3.95 & 2.3503 & 2.3001 & 2.7003 & 2.9503 \\
%y & 1.3501 & \cellcolor{gray!20} 3.3501 & 2.55 & \cellcolor{gray!20} 4.55 & 2.9502 & 2.9002 & \cellcolor{gray!20} 3.3002 & \cellcolor{gray!20} 3.2002\\ 
%z & 1.95 & \cellcolor{gray!20} 3.95 & .65 & 2.65 & 1.6502 & .6502 & 1.3002 & 1.6502\\
%$B^0$ & 1.95 & \cellcolor{gray!20}3.95 & 1.95 & \cellcolor{gray!20}3.95 & 2.9502 & 1.9502 & 2.6002 %& 2.9502 \\
%$B^1$ & 1.3501 & \cellcolor{gray!20} 3.3501 & 2.6 & \cellcolor{gray!20} 4.6 & \cellcolor{gray!20} 3.0502 & 2.6002 & \cellcolor{gray!20} 3.2502 & \cellcolor{gray!20} 3.3 \\
%B & 1.0001 & \cellcolor{gray!20} 3.0001 & 2.3001 & \cellcolor{gray!20} 4.3001 & 2.7002 & 2.3002 & 2.9502 & 2.9502\\




%x & .65 & 2.65 & 1.95 & 3.95 & 2.3503 & 2.3001 & 2.7003 & 3.0003 \\
%y & 1.3501 & 3.3501 & 2.55 & 4.55 & 2.9502 & 2.9002 & 3.3002 & 3.2002\\ 
%z & 1.95 & 3.95 & .65 & 2.65 & 3.002 & .6502 & 1.3002 & 1.6502\\
%$B^0$ & 1.95 & 3.95 & 1.95 & 3.95 & 3.7002 & 1.9502 & 2.6002 & 2.9502 \\
%$B^1$ & 1.3501 & 3.3501 & 2.6 & 4.6 & 3.0502 & 2.6002 & 3.2502 & 3.3 \\
%B & 1.0001 & 3.0001 & 2.3001 & 4.3001 & 2.7002 & 2.3002 & 2.9502 & 2.9502\\

